Contactless Cardiac Arrest Detection Using Smart Devices

Out-of-hospital cardiac arrest (OHCA) is a leading cause of death worldwide. Rapid diagnosis and initiation of cardiopulmonary resuscitation (CPR) is the cornerstone of therapy for victims of cardiac arrest. Yet a significant fraction of cardiac arrest victims have no chance of survival because they experience an unwitnessed event, often in the privacy of their own homes. An under-appreciated diagnostic element of cardiac arrest is the presence of agonal breathing, an audible biomarker and brainstem reflex that arises in the setting of severe hypoxia. Here, we demonstrate that a support vector machine (SVM) can classify agonal breathing instances in real-time within a bedroom environment. Using real-world labeled 9-1-1 audio of cardiac arrests, we train the SVM to accurately classify agonal breathing instances. We obtain an area under the curve (AUC) of 0.998 and an operating point with an overall sensitivity and specificity of 97.03% (95% CI: 96.62 -- 97.41%) and 98.20% (95% CI: 97.87 -- 98.49%). We achieve a false positive rate between 0% -- 0.10% over 82 hours (117,895 audio segments) of polysomnographic sleep lab data that includes snoring, hypopnea, central and obstructive sleep apnea events. We demonstrate the effectiveness of our contactless system in identifying real-world cardiac arrest-associated agonal breathing instances and successfully evaluate our classifier using commodity smart devices (Amazon Echo and Apple iPhone).

==> abstract-2.tex <==
\begin{sciabstract}
Out-of-hospital cardiac arrest (OHCA) is a leading cause of death worldwide. Rapid diagnosis and initiation of cardiopulmonary resuscitation (CPR) is the cornerstone of therapy for victims of cardiac arrest. Yet a significant fraction of cardiac arrest victims have no chance of survival because they experience an unwitnessed event, often in the privacy of their own homes. An under-appreciated  diagnostic element  of  cardiac arrest  is  the presence of agonal breathing, an audible biomarker and brainstem reflex that arises in the setting of severe hypoxia. Here, we demonstrate that a support vector machine (SVM) can classify agonal breathing instances in real-time within a bedroom environment. Using real-world labeled 9-1-1 audio of cardiac arrests, we train the SVM to accurately classify agonal breathing instances. We obtain an area under the curve (AUC) of 0.998 $\pm$ 0.004 and an operating point with an overall sensitivity and specificity of 97.03\% (95\% CI: 96.62 -- 97.41\%) and 98.20\% (95\% CI: 97.87 -- 98.49\%). We achieve a false positive rate between 0\% -- 0.10\% over 82 hours (117,895 audio segments) of polysomnographic sleep lab data that includes snoring, hypopnea, central and obstructive sleep apnea events. We demonstrate the effectiveness of our contactless system in identifying real-world cardiac arrest-associated agonal breathing instances and successfully evaluate our classifier using commodity smart devices (Amazon Echo and Apple iPhone).
\end{sciabstract}

==> abstract.tex <==
\begin{sciabstract}
% \begin{abstract}
Out-of-hospital cardiac arrest (OHCA) is a leading cause of death worldwide. Rapid diagnosis and initiation of cardiopulmonary resuscitation (CPR) is the cornerstone of therapy for victims of cardiac arrest. Yet a significant fraction of cardiac arrest victims have no chance of survival because they experience an unwitnessed event, often in the privacy of their own homes. An under-appreciated  diagnostic element  of  cardiac arrest  is  the presence of agonal breathing, an audible biomarker and brainstem reflex that arises in the setting of severe hypoxia. Here, we demonstrate that a support vector machine (SVM) can classify agonal breathing instances in real-time within a bedroom environment. Using real-world labeled 9-1-1 audio of cardiac arrests, we train the SVM to accurately classify agonal breathing instances. We obtain an area under the curve (AUC) of 0.998 $\pm$ 0.003 and an operating point with an overall sensitivity and specificity of 98.51\% (95\% CI: 98.21 -- 98.78\%) and 98.05\% (95\% CI: 97.71 -- 98.35\%). We achieve a false positive rate between 0\% -- 0.12\% over 83 hours (119,425 audio segments) of polysomnographic sleep lab data that includes snoring, hypopnea, central and obstructive sleep apnea events. We demonstrate the effectiveness of our contactless system in identifying real-world cardiac arrest-associated agonal breathing instances and successfully evaluate our classifier using commodity smart devices (Amazon Echo and Apple iPhone) \textcolor{red}{at distances of up to 6 m and in the presence of interfering indoor and outdoor sounds}.
% \end{abstract}
\end{sciabstract}

==> discussion-1.tex <==

In this report, we demonstrate that a neural network can accurately and efficiently classify agonal breathing, an audio biomarker of cardiac arrest. We deploy the classifier onto a commodity smartspeaker (Amazon Echo) and smartphone (iPhone 5s), both of which can accurately identify these unique sounds in real-time in an experimental setup using actual cardiac-arrest associated agonal breathing audio. 

Out-of-hospital cardiac arrest is a widespread public health concern. The treatment of cardiac arrest is well established, underscoring the vital importance of timely detection, followed by initiation of a series of time-dependent coordinated
actions which comprise the chain of survival\cite{neumar2015part}. Tens of thousands of people worldwide die annually from unwitnessed cardiac arrest, without any chance of survival because they are unable to have this chain of survival activated and receive timely resuscitation. Passive detection of agonal breathing potentially represents a novel way to identify a subset of previously unreachable victims of cardiac arrest, particularly those who experience such events in a private residence. As the US population ages and more people become at risk for OHCA, leveraging commodity smart hardware for surveillance of these emergent conditions could have public health benefits. The other domains where an efficient agonal breathing classifer could have utility is in unmonitored health facilities (hospital wards and elder care environments) as well as with 9-1-1 dispatchers to help more efficiently identify cardiac arrest during calls.

An immediate concern of a passive agonal breathing classifier is privacy.  For this use case, intentional activation of the device (i.e., "Hey Alexa" or "Hey Siri") prior to classification is not feasible because diagnosis involves an unconscious individual in an emergent situation. To address privacy concerns on smartphones, we designed our system to run locally; in the smart speaker implementation, a privacy preserving layer would be a necessary addition to our system. Such privacy preserving systems are an area of ongoing investigation\cite{larson2011accurate,liaqat2017method,chen2008audio}.

An advantage of a passive detection mechanism is that it does not require a victim to be wearing a device. A passive solution can also be implemented on existing wired smart speakers, and as a result would not face power constraints and could also scale efficiently. Potential downsides include that, to date, agonal breathing has been identified in approximately 50\% of cardiac arrest victims, so people experiencing an unwitnessed cardiac arrest without agonal breathing would go undetected by our system. Prior estimates of cardiac arrest-associated agonal breathing events have been based on 911 calls, which likely underestimates the true prevalence of agonal breathing during cardiac arrest. 

Another potential concern is the issue of potential false positives, given that a true positive classification should lead to activation of the emergency response system. Put differently, having a low false positive rate would be critical to manage public resources and avoid unnecessary deployment of EMS.  To further mitigate the risk of false-positives, we applied a heuristic in the second model based on breath spacing, which increased our specificity to 99.3\%. Additional agonal instances could help improve the specificity further, which would be required for a real-world implementation. A real-world implementation would also require a user-interface that had a confirmatory/cancellation opportunity before the emergency medical response system was activated.

There are limitations to this study and potential barriers to implementing an OHCA surveillance network based on agonal breathing. The number of agonal instances in this study was from one community over an 8-year period. Because of the rarity of this data, there exists the possibility that our models are over-fit. our dataset. We are optimistic that our proof-of-concept system and classifier would only improve with additional audio of agonal instances. {\bf using optimisitic seems werid} 


==> discussion-2.tex <==

In this report, we demonstrate that a neural network can accurately and efficiently classify agonal breathing, an audio biomarker of cardiac arrest. We evaluate the performance of our detector on a commodity smart speaker (Amazon Echo) and smartphone (iPhone 5s), both of which could accurately identify these unique sounds in experiments using actual cardiac-arrest associated agonal breathing audio. 

Out-of-hospital cardiac arrest is a widespread public health concern. Early CPR is a core treatment, underscoring the vital importance of timely detection, followed by initiation of a series of time-dependent coordinated
actions which comprise the chain of survival\cite{neumar2015part}. Hundreds of thousands of people worldwide die annually from unwitnessed cardiac arrest, without any chance of survival because they are unable to activate this chain of survival and receive timely resuscitation. Passive detection of agonal breathing represents a novel way to identify a portion of previously unreachable victims of cardiac arrest, particularly those who experience such events in a private residence. As the US population ages and more people become at risk for OHCA, leveraging commodity smart hardware for monitoring of these emergent conditions could have public health benefits. The other domains where an efficient agonal breathing detector could have utility is in unmonitored health facilities (hospital wards and elder care environments) as well as in assisting 9-1-1 dispatchers more efficiently identify cardiac arrest during 9-1-1 calls.

An immediate concern of a passive agonal breathing detector is privacy.  For this use case, intentional activation of the device (i.e., "Hey Alexa" or "Hey Siri") prior to classification is not feasible because diagnosis involves an unconscious individual in an emergent situation. To address privacy concerns on smartphones, we designed our system to run locally; in the smart speaker implementation, a privacy preserving layer would be a necessary addition to our system. Such privacy preserving systems are an area of ongoing investigation\cite{larson2011accurate,liaqat2017method,chen2008audio}.

An advantage of a passive detection mechanism is that it does not require a victim to be wearing a device. A passive solution can also be implemented on existing wired smart speakers, and as a result would not face power constraints and could scale efficiently. Potential downsides include that, to date, agonal breathing has been identified in approximately 50\% of cardiac arrest victims, so people experiencing an unwitnessed cardiac arrest without agonal breathing would go undetected by our system. Prior estimates of cardiac arrest-associated agonal breathing events have been based on 911 calls, which likely biases estimates and underestimates the true prevalence of agonal breathing during cardiac arrest.\cite{bobrow2008gasping}

There are limitations to this study and potential barriers to implementing an OHCA monitoring system triggered by agonal breathing. The number of agonal instances in this study was from one geographic community over an 8-year period. Additional agonal events are needed to assure our model generalizes to variations of agonal breathing. Additional audio of agonal instances, which likely reside in 911 databases around the world, would also contribute to a more accurate detection system. Finally, it is not known if conditions such as seizure, hypoglycemia, severe stroke or drug overdoses with disordered breathing (but not agonal breathing) could be distinct or similar to agonals and thus could pose a challenge to classification. Further work is needed in this area, yet all of these instances represent acute conditions requiring prompt medical intervention.

Technology is rapidly evolving and in turn providing opportunities to improve human health.\cite{gambhir2018toward,steinhubl2015emerging} The increasing adoption of commodity smart speakers in private residences \cite{gartner} and hospital environments\cite{specialreport} may provide a wide-reaching means to realize the potential of a passive cardiac arrest detection system.


==> intro-2.tex <==
Out-of-hospital cardiac arrest (OHCA) is a leading cause of death worldwide\cite{myat2018out} and in North America accounts for nearly 300,000 deaths annually.\cite{mcnally2011out} The treatment of cardiac arrest, cardiopulmonary resuscitation (CPR), is well established and its effectiveness is time-dependent\cite{field2010part}, with survival decreasing by 7-10 percent for every minute that passes without administration of CPR\cite{larsen1993predicting}.

 One diagnostic element of cardiac arrest is the presence of a distinctive type of disordered breathing: agonal breathing.\cite{graham2015strategies,rea2005agonal} Agonal breathing, which arises from a brainstem reflex in the setting of severe hypoxia\cite{poets1999gasping,lumsden1923observations}, appears to be evident in approximately half of cardiac arrest cases reported to 9-1-1 and its presence has been associated with favorable neurological outcomes.\cite{clark1992incidence,baang2003interaction} Typically reported as ``gasping" respirations, agonal respirations may hold underexplored potential as an audible diagnostic biomarker, particularly in unwitnessed cardiac arrests that occur in a private residence, the location of 75 percent of such unwitnessed emergencies\cite{xxx}.

The widespread adoption of smartphones and smart speakers (projected to be in 75\% of US households by 2020\cite{gartner}) present a unique opportunity to identify this audible biomarker and connect unwitnessed cardiac arrest victims to Emergency Medical Services (EMS) and CPR. In this study, we hypothesized that existing commodity devices (e.g., smartphones and smart speakers) could be used to accurately identify OHCA-associated agonal breathing instances. A key challenge to algorithm development for this purpose is accessing real-world data on agonal breathing, which is extraordinarily difficult; agonal events are rare, lack gold-standard measurements and cannot be reproduced in a lab because of their emergent nature. We overcome this challenge by using a unique data source, 9-1-1 audio of confirmed cardiac arrest cases, which can include agonal breathing instances captured during the call. Using real-world audio of agonal instances from witnessed cardiac arrest events, we evaluate (1) whether a Deep Neural Network (DNN) can be trained to accurately classify OHCA-associated agonal breathing instances and (2) whether the neural network can be deployed and accurately classify agonal breathing audio in real-time on existing commodity smart speakers and smartphones.

\textcolor{red}{SHYAM: I would remove this para} Interventions that reduce the time from OHCA diagnosis to CPR initiation, particularly in unwitnessed settings, may hold potential for reducing morbidity and mortality.\cite{weaver1986factors,cummins1985survival} Because unwitnessed cardiac arrest victims have no chance of survival without immediate detection and initiation of CPR, a widely available real-time sensing system, capable of signaling to EMS or nearby bystanders, may hold potential to improve survivability of unwitnessed cardiac arrest. 

==> intro-3.tex <==
% \section*{Introduction}



Out-of-hospital cardiac arrest (OHCA) is a leading cause of death worldwide\cite{myat2018out} and in North America accounts for nearly 300,000 deaths annually.\cite{mcnally2011out} A relatively under-appreciated diagnostic element of cardiac arrest is the presence of a distinctive type of disordered breathing: agonal breathing.\cite{graham2015strategies,rea2005agonal} Agonal breathing, which arises from a brainstem reflex in the setting of severe hypoxia\cite{poets1999gasping,lumsden1923observations}, appears to be evident in approximately half of cardiac arrest cases reported to 9-1-1. Agonal breathing indicates a relatively short duration of collapse and has been associated with higher survival rates, though agonal breathing can also confuse the rescuer or 9-1-1 operator about the nature of the illness.\cite{hauff2003factors,clark1992incidence,baang2003interaction} Sometimes reported as ``gasping" breaths, agonal respirations may hold potential as an audible diagnostic biomarker, particularly in unwitnessed cardiac arrests that occur in a private residence, the location of 2/3 of all OHCAs.\cite{van2017multistate}

The widespread adoption of smartphones and smart speakers (projected to be in 75\% of US households by 2020\cite{gartner}) present a unique opportunity to identify this audible biomarker and connect unwitnessed cardiac arrest victims to Emergency Medical Services (EMS) and cardiopulmonary resuscitation (CPR). In this study, we hypothesized that existing commodity devices (e.g., smartphones and smart speakers) could be used to accurately identify OHCA-associated agonal breathing instances. A key challenge to algorithm development for this purpose is accessing real-world data on agonal breathing; agonal breathing events are relatively uncommon, lack gold-standard measurements and cannot be reproduced in a lab because of their emergent nature. To overcome this challenge, we leverage a unique data source, 9-1-1 audio of confirmed cardiac arrest cases, which can include agonal breathing instances captured during the call. Using real-world audio of agonal instances from OHCA events, we evaluate (1) whether a Deep Neural Network (DNN) can be trained to accurately classify OHCA-associated agonal breathing instances and (2) whether the neural network can be deployed and accurately classify agonal breathing audio in real-time on existing commodity smart speakers and smartphones.


==> methods-1.tex <==
\section*{Materials and methods}
\subsection{Datasets.}

This study was approved by the University of Washington Institutional Review Board (STUDY00004839). Data were provided by Public Health--Seattle \& King County, division of Emergency Medical Services. The data represent the subset of 9-1-1 calls which (a) contained a known cardiac arrest and (b) had been identified by a research assistant (a trained 9-1-1 dispatcher) to contain cardiac arrest-associated agonal breathing instances.

\subsection{Data preparation.} The agonal breathing instances were extracted from the 9-1-1 emergency calls, with each audio clip lasting 2.5 seconds. We only extracted clear instances of agonal breathing that did not co-occur with other interfereing sounds. We note that the audio clips were sampled at a frequency of 8~kHz which is standard for audio received over a telephone. The audio clips were then converted into a spectrogram with a 448-point Fast Fourier Transform Hamming window size of 188 samples, 100 samples that overlap between time segments. The resultant power values are converted into decibels, and each power value is mapped to the jet colormap in Matlab, where red and blue values represented high and low power intensities respectively. The spectrogram is then resized to be a 224 by 224 image so it is compatible as an input to our neural network.

\subsection{Training algorithm.} The dataset to train and validate our model for detecting unwitnessed agonal breathing contains 236 agonal breathing recordings and 1590 non-agonal audio segments from the 911 calls, sampled uniformly across each of the calls. The model for detecting agonal breathing in 9-1-1 calls uses 400 non-agonal breathing recordings from sampled uniformly across 8 audio event categories from Google's AudioSet, namely ambient noise, snoring, human speech, sounds from a TV or radio, cat or dog sounds, fan or aircon sounds, coughing and breathing. We use k-fold (k=10) validation to estimate the performance of both models. Each 9-1-1 call in our dataset contains on average 2 clearly heard agonal breathing instances. To reduce bias in our classifier we partitioned the data such that recordings from the same call did not straddle the training and validation set split. We set the target number positive recordings in our validation set size to be 22 samples for each validation fold, approximately 10\% of the 236 agonal breathing recordings.

We use the MobileNet CNN which has been pretrained on the ImageNet dataset of 1000 object categories to have a top-5 accuracy of 89.5\%. To adapt the CNN to our agonal breathing detection task, we remove the final classification layer and replace it with a fully-connected layer containing 256 nodes followed by Dropout\cite{dropout} with a rate of 0.6 and a fully-connected layer with 2 nodes and a softmax activation. These final layers are trained using transfer learning using RMSProp with a learning rate of 0.00001. Due to the class imbalance between positive and negative audio segments, we proportionally bias the classifier to place a higher value on correctly classifying positive audio segments of agonal breathing.

\subsection{Classifier Performance.} When testing our model for 9-1-1 calls across 12 hours of non-agonal breathing segments we only considered pairs of positively marked segments and that occurred within 30 seconds of each other to be indicative of agonal breathing. This mitigates the effects of spurious false positives. We found that on average, instances of agonal breathing in our dataset were separated by 30 seconds of negative sounds, which is due to the nature of our dataset. For many of the calls, agonal breathing is only recorded when the operator instructs the callee to hold the phone close to the agonal breather, and is not heard for the rest of the call. The occurrences of agonal breathing is mostly dependent on the callee's distance to the agonal breather, which would vary over time, and whether or not the phone was in speakerphone mode, as opposed to the actual frequency of agonal breathing. In our proposed use case of a static smart speaker or smartphone agonal breathing would typically be heard more than two times within a 30 second time frame. The selection of a 30 second gap is conservative enough that it can substantially reduce false positives, but also short enough so as not to unacceptably delay signaling Emergency Medical Services.

To obtain the classifier performance for each negative audio event category, we set the negative recordings within a given validation set to be a) from a single category and b) equal to the number of positive recordings by using additional data from AudioSet that was not used during the training phase. We then obtain an ROC curve and corresponding AUC for each negative category (Figure \ref{fig:rocs}).

\subsection{Benchmark Performance.} We benchmark the classifier's performance in several benchmark scenarios. The model trained and validated on the original 9-1-1 calls and AudioSet recordings are used to evaluate the audio clips recorded for the different benchmark scenarios.

Figure \ref{fig:bm}A shows the detection accuracy of our classifier across different distances on a second generation Amazon Echo and an iPhone 5s. We played the 236 audio clips of agonal breathing from a AmazonBasics Wireless Bluetooth speaker and recorded the audio on the Echo and iPhone. The sound intensity of the recordings were approximately 70 dBA at a distance of 1 meter. We fixed the location of the Echo and iPhone and placed the speaker at different distances.

To record audio indefinitely on the Echo we used Echo's Drop In feature which streams audio to another smartphone. That smartphone was plugged into a laptop which recorded audio data that was received on the smartphone's audio interface. Audio from the Echo is streamed at 16 kHz and recorded at 44.1 kHz. The iPhone recorded data at 44.1 kHz.

Each of the 236 audio clips is prepended with a frequency modulated continuous wave (FMCW) chirp. An FMCW chirp has good autocorrelation properties, as a result we can cross-correlate the recordings from the Echo and iPhone with the chirp to determine the exact time stamp of each audio clip. Each audio clip can then be extracted and transformed into an input for the neural network.

The results show that both devices achieve close to ideal detection across distances of 1 to 6 meters. Detection accuracies start to decrease gradually for for both devices. At a distance of 14 meters, the Echo and smartphone have an accuracy of 78.4\% $\pm$ 5.8\% and 91.6\% $\pm$ 6.72\% respectively.

Next we evaluate the effect of an obstructing door on our detection accuracy. We repeat the same experiment as above but place a wooden door in between the speaker and our recorders. Figure \ref{fig:bm}B shows high accuracies ($>$ 95\%) for both devices at distances of 1 to 3 meters. Detection accuracies drop off quickly and the audio clips are close to undetectable at 14 meters. The range of 1 -- 3 meters may be sufficient in situations where the agonal breathing event and recording device are in adjacent rooms such as a bedroom and ensuite bathroom.

We also evaluated the effect of placing the smartphone in a pocket and obtain a detection accuracy of 97.4\% $\pm$ 3.5\%.

Figure \ref{fig:bm}C shows our system performance in the presence of 6 classes of interfering sounds, namely fan and aircon sounds, human speech, cat and dog sounds, music and shower sounds. In this experiment we use two external speakers, one which plays the agonal breathing recordings and another that plays the interfereing noise. Both speakers are placed 3 meters away from the recording devices and perpendicular to each other with respect to the recording devices. The interfereing noise is played at a similar volume to the agonal breathing recordings. Across all interfering sounds classes the smart speaker and smartphone both achieve a detection accuracy of at least 91\%.

Finally we evaluate the system performance when the source of the audio interference is the recording device itself. To do this we set the iPhone 5s to play music at a louder volume (85 dBA at a distance of 1 meter) than the agonal breathing audio clips, while simultaneously recording audio. 

We then ran an acoustic interference cancellation algorithm that allowed the smartphone to locally reduce the interference of its own audio transmissions. We used an adaptive least mean squares filter to reduce the dissimilarity between the device's transmission and the received audio recording. Our filter uses the Matlab implementation of the Sign-Data LMS algorithm with 100 weights and a step size of 0.05.

Without any audio cancellation, the detection accuracy is consistently poor, with an average accuracy of 9.5\% across distances. When the audio cancellation algorithm is applied, our detection accuracy improves to 97.0\% $\pm$ 3.4\% at a distance of 1 meter, and gradually decreases to an accuracy of 74.9\% $\pm$ 15.4\% at 14 meters.

\subsection{Run-time Analysis.} Our iPhone implementation of the detection algorithm used the Accelerate frameworks to perform the FFTs required to generate the spectrogram and the CoreML framework to run neural network inferences. On an iPhone 7 performing the FFTs to generate a single spectrogram takes 35 ms and running inferences on the neural network takes 32 ms. 


==> methods-2.tex <==
\section*{Materials and methods}
\subsection{Datasets.}

This study was approved by the University of Washington Institutional Review Board. Data were provided by Public Health--Seattle \& King County, Division of Emergency Medical Services. The data represent a subset of 9-1-1 calls which (a) contained a known cardiac arrest and (b) had been identified by a research assistant (a trained 9-1-1 dispatcher) to contain cardiac arrest-associated agonal breathing instances.

\subsection{Data preparation.} The agonal breathing instances extracted from the 9-1-1 emergency calls were manually filtered to only contain clear instances of agonal breathing that did not co-occur with other interfering sounds. We note that the audio clips were sampled at a frequency of 8~kHz which is standard for audio received over a telephone. All audio clips were normalized to have a mean of zero. The audio clips were then converted into a spectrogram with a 448-point Fast Fourier Transform Hamming window size of 188 samples, 100 samples that overlap between time segments. The resultant power values are converted into decibels, and each power value is mapped to the jet colormap in Matlab with a maximum and minimum power spectral density of -150 and -50 dB/Hz respectively. Red and blue values represented high and low power intensities respectively. The spectrogram is then resized to be a 224 by 224 image so it is compatible as an input to our neural network.

\subsection{Training algorithm.} The dataset to train and validate our model for detecting unwitnessed agonal breathing contains 236 agonal breathing recordings and 1590 non-agonal audio segments from the 911 calls, sampled uniformly across each of the calls. The model for detecting agonal breathing in 9-1-1 calls uses 400 non-agonal breathing recordings sampled uniformly across 8 audio event categories from Google's AudioSet. These sounds include ambient noise, snoring, human speech, sounds from a TV or radio, cat or dog sounds, fan or aircon sounds, coughing and breathing. Each 9-1-1 call in our dataset contains on average 2 clearly heard agonal breathing instances. To reduce bias in our classifier we partitioned the data such that recordings from the same call did not straddle the training and validation set split. We set the target number positive recordings in our validation set size to be 22 samples for each validation fold, approximately 10\% of the 236 agonal breathing recordings.

We use the MobileNet CNN which has been pretrained on the ImageNet dataset of 1000 object categories to have a top-5 accuracy of 89.5\%. To adapt the CNN to our agonal breathing detection task, we remove the final classification layer and replace it with a fully-connected layer containing 256 nodes followed by Dropout\cite{dropout} with a rate of 0.6 and a fully-connected layer with 2 nodes and a softmax activation. These final layers resulted in 12,845,826 parameters and were trained using transfer learning using RMSProp with a learning rate of 0.00001. Due to the class imbalance between positive and negative audio segments, we proportionally bias the classifier to place a higher value on correctly classifying positive audio segments of agonal breathing.

\subsection{Classifier Performance.} When testing our model for 9-1-1 calls across 12 hours of non-agonal breathing segments we only considered pairs of positively marked segments and that occurred within 30 seconds of each other to be indicative of agonal breathing. We found that on average, instances of agonal breathing in our dataset were separated by 30 seconds of negative sounds, which is due to the nature of our dataset. For many of the calls, agonal breathing is only recorded when the operator instructs the callee to hold the phone close to the agonal breather, and is not heard for the rest of the call. The occurrences of agonal breathing is mostly dependent on the callee's distance to the agonal breather, which would vary over time, and whether or not the phone was in speakerphone mode, as opposed to the actual frequency of agonal breathing. In our proposed use case of a static smart speaker or smartphone agonal breathing would typically be heard more than two times within a 30 second time frame. The selection of a 30 second gap is conservative enough that it can substantially reduce false positives, but also short enough so as not to unacceptably delay signaling Emergency Medical Services.

\subsection{Benchmark Performance.} In our benchmark scenarios we evaluate the detection accuracy of our classifier across different distances on a second generation Amazon Echo and an iPhone 5s. We played the 236 audio clips of agonal breathing from a AmazonBasics Wireless Bluetooth speaker and recorded the audio on the Echo and iPhone. The sound intensity of the recordings were approximately 70 dBA at a distance of 1 meter. We fixed the location of the Echo and iPhone and placed the speaker at different distances.

To record audio indefinitely on the Echo we used Echo's Drop In feature which streams audio to another smartphone. That smartphone was plugged into a laptop which recorded audio data that was received on the smartphone's audio interface. Audio from the Echo is streamed at 16 kHz and recorded at 44.1 kHz. The iPhone recorded data at 44.1 kHz.

Each of the 236 audio clips is prepended with a frequency modulated continuous wave (FMCW) chirp. An FMCW chirp has good autocorrelation properties, as a result we can cross-correlate the recordings from the Echo and iPhone with the chirp to determine the exact time stamp of each audio clip. Each audio clip can then be extracted and transformed into an input for the neural network.

When evaluating system performance in the presence of interfering sounds we use two external speakers, one which plays the agonal breathing recordings and another that plays the interfering noise. Both speakers are placed 3 meters away from the recording devices and perpendicular to each other with respect to the recording devices. The interfering noise and agonal breathing sounds are played with a sound intensity of approximately 70 dBA at a distance of 1 meter.

To evaluate the audio interference cancellation algorithm we set the iPhone 5s to play music at a louder volume (85 dBA at a distance of 1 meter) than the agonal breathing audio clips, while simultaneously recording audio. 

We then ran an acoustic interference cancellation algorithm that allowed the smartphone to locally reduce the interference of its own audio transmissions. We used an adaptive least mean squares filter to reduce the dissimilarity between the device's transmission and the received audio recording. Our filter uses the Matlab implementation of the Sign-Data LMS algorithm with 100 weights and a step size of 0.05.

\subsection{Run-time Analysis.} Our iPhone 7 implementation of the detection algorithm used the Accelerate frameworks to perform the FFTs required to generate the spectrogram and the CoreML framework to run neural network inferences. On an iPhone 7 performing the FFTs to generate a single spectrogram takes 60 ms and running inferences on the neural network takes 30 ms.

To estimate the performance of our system when run natively on an Amazon Echo, we ran our pipeline on an iPhone 4, which shares the same Cortex-A8 processor as the Echo. On an iPhone 4, computing the spectrogram takes 100 ms and running inferences the neural network takes 45 ms.

% Computing the spectrogram takes on average 100 ms and this was estimated with an implementation on an iPhone 4, which uses the Cortex-A8 processor used in the first-generation Alexa\cite{ifixit}. 

% By profiling the execution sequence of the MobileNet architecture in Tensorflow, we find that a single inference requires running 1.1 million floating point operations. Our system does inferences every 2.5 seconds, which translates to 458 MFLOPS (floating point operations per second). The Alexa Voice Service Development Kit uses Cortex-A7 processors that have an execution speed of 1000 MCPS (cycles per second)\cite{devkit}. The Cortex-A7 executes 1 double precision FLOP per cycle \cite{cortex}, as a result it is able to execute a single neural network inference in 458 ms. The pipeline is thus able to run within 558 ms which is within the time constraint of 2.5 seconds. 


==> methods-3.tex <==
\section*{Materials and methods}

This study was approved by the University of Washington Institutional Review Board. Data were provided by Public Health--Seattle \& King County, Division of Emergency Medical Services.

\subsection{Datasets.}
The data represents a subset of 9-1-1 calls which (a) contained a known cardiac arrest and (b) had been identified  to contain cardiac arrest-associated agonal breathing instances. The negative data consists of recordings of 12 patients sleeping in a sleep lab recorded on a Samsung Galaxy S4.

{Our agonal breathing recordings are sourced from 9-1-1 emergency calls from 2009--2017 provided by Public Health--Seattle \& King County, Division of Emergency Medical Services. There are 729 calls totaling to 82 hours. The provided recordings include only calls involving cardiac arrest and specifically those determined to contain occurrences of agonal breathing, either by audible identification of agonal breathing or by description of the breathing from the caller. Each call is further rated by the 9-1-1 operator and a quality assurance reviewer with a confidence score indicating the presence of audible agonal instances. We train our classifier on audio from calls that are rated with high confidence by both the operator and reviewer to contain audible agonal instances. A trained researcher then listened to the 162 calls (19 hours) meeting these criteria and manually recorded timestamps where agonal breathing was  heard during the call (see Supplementary Table 1).  These instances predominantly occur when the 9-1-1 operator asks the caller to place the phone next to the victim's mouth for the purposes of breathing identification. For every timestamp annotation, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances.}


Our negative dataset consists of 83 hours of audio from polysomnographic studies across 12 different patients and contains instances of hypopnea, central apnea, obstructive apnea, snoring and breathing. The female to male ratio was 0.5 and the median age was 57.0 (IQR: 11.5). The mean number of hypopnea, central apnea and obstructive apnea events across patients was 41, 24 and 26 respectively. The mean apneas-hypopneas index (AHI) is 13, where a value of 0-5 is considered as no apnea, 5-15 is considered as mild apnea and 15-30 is considered as moderate apnea, higher values are considered as severe apnea\cite{nieto2000association}. These annotations were provided by trained sleep technicians. The negative dataset also includes interfering sounds that might be played while a person is asleep: podcast, sleep soundscape and white noise. 


Given the relatively small size of our agonal breathing dataset, we augmented the number of agonal breathing instances with label preserving transformations, a common technique applied to sparse datasets\cite{cui2015data,wong2016understanding}. We augment the data by playing the recordings over the air over distances of 1, 3 and 6 meters, in the presence of interference from indoor and outdoor sounds with different volumes and when a noise cancellation filter is applied. The recordings were captured on different devices, namely an Amazon Alexa, an iPhone 5s and a Samsung Galaxy S4. Similarly, for the negative dataset, portions of the sleep data from all patients were played over the air and recorded on different devices as well as over a phone connection. We play a five minute portion of audio data from each patient over the air at different distances and record the data on an Amazon Alexa, iPhone 5s and over a phone connection.  The entire dataset for cross-validation consists of 14,655 data points with 7316 agonal breathing instances and 7339 instances of negative data. 

\subsection{Data preparation.} We note that the audio clips were sampled at a frequency of 8~kHz which is standard for audio received over a telephone. All audio clips are normalized between a range of -1 and 1. The audio clips are then passed through Google's VGGish\cite{vggish} model for extracting feature embeddings from an audio waveform. The VGGish model transforms the waveforms into a compact embedding. The model resamples all audio waveforms at 16 kHz then computes a spectrogram using the Short-Time Fourier Transform. A log mel spectrogram is generated and PCA is applied on the spectrogram to produce a 256-dimensional embedding.

\subsection{Training algorithm.}  We performed k-fold validation (k=10). For any given fold, none of the breathing instances in the validation set occurred in the training set. We evaluate detection accuracy such that no audio file in the validation set appears in any of the different recording conditions in the training set (e.g. if a file played at 6 m is present in the validation set, the same file played at 1 m is not present in the training set). We use a support vector machine with a radial basis function kernel and a regularization (C parameter) of 10 .To reduce bias in our classifier we partitioned the data such that recordings from the same call did not straddle the training and validation set split. 

\subsection{Benchmark experiments.}  To record audio indefinitely on the Echo we used Echo's Drop In feature which streams audio to another smartphone. That smartphone was plugged into a laptop which recorded audio data that was received on the smartphone's audio interface. Audio from the Echo is streamed at 16 kHz and recorded at 44.1 kHz. The iPhone recorded data at 44.1 kHz. Each of the 236 audio clips is prepended with a frequency modulated continuous wave (FMCW) chirp. An FMCW chirp has good auto-correlation properties, as a result we can cross-correlate the recordings from the Echo and iPhone with the chirp to determine the exact time stamp of each audio clip. Each audio clip can then be extracted and transformed into an input for the classifier.

In our benchmark scenarios we evaluate the detection accuracy of our classifier across different distances on a second generation Amazon Echo and an iPhone 5s. We played the 236 audio clips of agonal breathing from a AmazonBasics Wireless Bluetooth speaker and recorded the audio on the Echo and iPhone. The sound intensity of the recordings were approximately 70 dBA at a distance of 1 meter. We fixed the location of the Echo and iPhone and placed the speaker at different distances.  



To evaluate the audio interference cancellation algorithm we set the iPhone 5s to play music at two different volumes (45 and 67 dBA), while simultaneously recording audio. We then ran an acoustic interference cancellation algorithm that allowed the smartphone to locally reduce the interference of its own audio transmissions. We used an adaptive least mean squares filter to reduce the dissimilarity between the device's transmission and the received audio recording. Our filter uses the Sign-Data LMS algorithm with 100 weights and a step size of 0.05.


When evaluating system performance in the presence of interfering sounds we use two external speakers, one which plays the agonal breathing recordings and another that plays the interfering noise. The interfering noise is played with a sound intensity of approximately 55 dBA at a distance of 1 meter. 
The interfering sounds are played outside the room containing the agonal breathing speaker and the recording device to simulate sounds that would be heard from outside a bedroom. 




\subsection{Run-time Analysis.}  The most time consuming operations within the detection pipeline are the Fast Fourier Transforms (FFTs) required to generate the spectrogram and running inferences on the audio embeddings. Our iPhone 7 implementation of the detection algorithm used the Accelerate frameworks to perform the FFTs and Monte Carlo sampling to approximate the radial basis function kernel. On an iPhone 7 performing the FFTs to generate a single log mel spectrogram takes 16 ms and running inferences on the support vector machine takes 5 ms. While the classifier can in principle run locally on the Echo device, Amazon currently does not allow third party programs to locally analyse data. Thus, to estimate the performance of our system when run natively on an Amazon Echo, we ran our pipeline on an iPhone 4, which shares the same Cortex-A8 processor as the Echo. On an iPhone 4, computing the spectrogram takes 40 ms and making predictions takes 18 ms.

t

==> methods-npj.tex <==
\section*{Materials and methods}

This study was approved by the University of Washington Institutional Review Board. Data were provided by Public Health--Seattle \& King County, Division of Emergency Medical Services.

\subsection*{Datasets.}
The data represents a subset of 9-1-1 calls which (a) contained a known cardiac arrest and (b) had been identified  to contain cardiac arrest-associated agonal breathing instances. The negative data consists of recordings of 12 patients sleeping in a sleep lab recorded on a Samsung Galaxy S4.

{Our agonal breathing recordings are sourced from 9-1-1 emergency calls from 2009--2017 provided by Public Health--Seattle \& King County, Division of Emergency Medical Services. There are 729 calls totaling to 82 hours. The provided recordings include only calls involving cardiac arrest and specifically those determined to contain occurrences of agonal breathing, either by audible identification of agonal breathing or by description of the breathing from the caller. Each call is further rated by the 9-1-1 operator and a quality assurance reviewer with a confidence score indicating the presence of audible agonal instances. We train our classifier on audio from calls that are rated with high confidence by both the operator and reviewer to contain audible agonal instances. These instances predominantly occur when the 9-1-1 operator asked the caller to place the phone next to the victim's mouth for the purposes of breathing identification. A trained researcher then listened to the 162 calls (19 hours) meeting these criteria and manually recorded timestamps where agonal breathing was  heard during the call (see Supplementary Table 1).  These instances predominantly occur when the 9-1-1 operator asks the caller to place the phone next to the victim's mouth for the purposes of breathing identification. For every timestamp annotation, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances.}


Our negative dataset consists of 83 hours of audio from polysomnographic studies across 12 different patients and contains instances of hypopnea, central apnea, obstructive apnea, snoring and breathing. The female to male ratio was 0.5 and the median age was 57.0 (IQR: 11.5). The mean number of hypopnea, central apnea and obstructive apnea events across patients was 41, 24 and 26 respectively. The mean apneas-hypopneas index (AHI) is 13, where a value of 0-5 is considered as no apnea, 5-15 is considered as mild apnea and 15-30 is considered as moderate apnea, higher values are considered as severe apnea\cite{nieto2000association}. These annotations were provided by trained sleep technicians. The negative dataset also includes interfering sounds that might be played while a person is asleep: podcast, sleep soundscape and white noise. 


We augmented the number of agonal breathing instances with label preserving transformations, a common technique applied to sparse datasets\cite{cui2015data,wong2016understanding}. We augment the data by playing the recordings over the air over distances of 1, 3 and 6 meters, in the presence of interference from indoor and outdoor sounds with different volumes and when a noise cancellation filter is applied. The recordings were captured on different devices, namely an Amazon Alexa, an iPhone 5s and a Samsung Galaxy S4. Similarly, for the negative dataset, portions of the sleep data from all patients were played over the air and recorded on different devices as well as over a phone connection. We play a five minute portion of audio data from each patient over the air at different distances and record the data on an Amazon Alexa, iPhone 5s and over a phone connection.  The entire dataset for cross-validation consists of 14,655 data points with 7316 agonal breathing instances and 7339 instances of negative data. 

\subsection*{Data preparation.} We note that the audio clips were sampled at a frequency of 8~kHz which is standard for audio received over a telephone. All audio clips are normalized between a range of -1 and 1. The audio clips are then passed through Google's VGGish\cite{vggish} model for extracting feature embeddings from an audio waveform. The VGGish model transforms the waveforms into a compact embedding. The model resamples all audio waveforms at 16 kHz then computes a spectrogram using the Short-Time Fourier Transform. A log mel spectrogram is generated and PCA is applied on the spectrogram to produce a 256-dimensional embedding.

\subsection*{Training algorithm.}  We performed k-fold validation (k=10). For any given fold, none of the breathing instances in the validation set occurred in the training set. We evaluate detection accuracy such that no audio file in the validation set appears in any of the different recording conditions in the training set (e.g. if a file played at 6 m is present in the validation set, the same file played at 1 m is not present in the training set). We use a support vector machine with a radial basis function kernel and a regularization (C parameter) of 10. To reduce bias in our classifier we partitioned the data such that recordings from the same call did not straddle the training and validation set split. 

\subsection*{Benchmark experiments.}  To record audio indefinitely on the Echo we used Echo's Drop In feature which streams audio to another smartphone. That smartphone was plugged into a laptop which recorded audio data that was received on the smartphone's audio interface. Audio from the Echo is streamed at 16 kHz and recorded at 44.1 kHz. The iPhone recorded data at 44.1 kHz. Each of the 236 audio clips is prepended with a frequency modulated continuous wave (FMCW) chirp. An FMCW chirp has good auto-correlation properties, as a result we can cross-correlate the recordings from the Echo and iPhone with the chirp to determine the exact time stamp of each audio clip. Each audio clip can then be extracted and transformed into an input for the classifier.

In our benchmark scenarios we evaluate the detection accuracy of our classifier across different distances on a second generation Amazon Echo and an iPhone 5s. We played the 236 audio clips of agonal breathing from a AmazonBasics Wireless Bluetooth speaker and recorded the audio on the Echo and iPhone. The sound intensity of the recordings were approximately 70 dBA at a distance of 1 meter. We fixed the location of the Echo and iPhone and placed the speaker at different distances.  



To evaluate the audio interference cancellation algorithm we set the iPhone 5s to play music at two different volumes (45 and 67 dBA), while simultaneously recording audio. We then ran an acoustic interference cancellation algorithm that allowed the smartphone to locally reduce the interference of its own audio transmissions. We used an adaptive least mean squares filter to reduce the dissimilarity between the device's transmission and the received audio recording. Our filter uses the Sign-Data LMS algorithm with 100 weights and a step size of 0.05.


When evaluating system performance in the presence of interfering sounds we use two external speakers, one which plays the agonal breathing recordings and another that plays the interfering noise. The interfering noise is played with a sound intensity of approximately 55 dBA at a distance of 1 meter. 
The interfering sounds are played outside the room containing the agonal breathing speaker and the recording device to simulate sounds that would be heard from outside a bedroom. 




\subsection*{Run-time Analysis.}  The most time consuming operations within the detection pipeline are the Fast Fourier Transforms (FFTs) required to generate the spectrogram and running inferences on the audio embeddings. Our iPhone 7 implementation of the detection algorithm used the Accelerate frameworks to perform the FFTs and Monte Carlo sampling to approximate the radial basis function kernel. On an iPhone 7 performing the FFTs to generate a single log mel spectrogram takes 16 ms and running inferences on the support vector machine takes 5 ms. While the classifier can in principle run locally on the Echo device, Amazon currently does not allow third party programs to locally analyse data. Thus, to estimate the performance of our system when run natively on an Amazon Echo, we ran our pipeline on an iPhone 4, which shares the same Cortex-A8 processor as the Echo. On an iPhone 4, computing the spectrogram takes 40 ms and making predictions takes 18 ms.



==> results-1.tex <==
Our detection algorithm is designed to identify the presence of agonal breathing in audio captured by a smart speaker or smartphone in real-time. Our system continuously makes predictions on audio segments with a duration of 2.5 seconds which is sufficient for reliably capturing an agonal breath (Figure \ref{fig:sig}A). Each segment is transformed from the time-domain into a spectrogram (Figure \ref{fig:sig}B) which visually represents the power spectral density of the signal, which is the power of each frequency in the audio segment as a function of time. The spectrogram image is then passed into a deep neural network that can distinguish between agonal breathing instances (positive data) and non-agonal instances (negative data). The negative data in this report include non-agonal portions of the 9-1-1 audio and other audio event categories which may be present in a private residence: ambient noise, snoring, human speech, sounds from a TV or radio, cat or dog sounds, fan or air conditioner sounds, coughing and normal breathing. These categories reflect typical sounds that might be heard in a domestic setting where only 1 person is present. The negative data is sourced from Google's AudioSet\cite{audioset} dataset which contains audio clips from YouTube spanning over 600 audio event classes.

We use the MobileNet\cite{mobilenet} CNN architecture that has been pretrained on the ImageNet dataset containing over a 1000 object classes. Using transfer learning\cite{tlearning} we adapt the weights of the convolutional neural network to the task of agonal breathing detection. Our detection algorithm can run in real-time on a smartphone and classify each 2.5 second audio segment in 67 ms.

We visually investigate the features learned by our neural network. First, we used LIME\cite{lime} to highlight the regions of a spectrogram that contribute most to the neural network's predictions. Figure \ref{fig:sig}C shows a masked spectrogram of agonal breathing. There is a correlation between the regions where agonal breathing occurs and the pixels that the classifier deems most important. Second, we applied t-SNE\cite{tsne} to visualize the high-dimensional outputs of the CNN's final hidden layer by projecting the features into the 2-D space (Figure \ref{fig:sig}D). The two clusters represent the abstract features of the agonal breathing and non-agonal breathing spectrograms for a subset of the non-agonal breathing sounds. 

We obtained recordings of 9-1-1 emergency calls from our local emergency medical service center that contained occurrences agonal breathing from 2009 -- 2017. The entire dataset contains 729 calls totalling to 82 hours. During most calls the operator would ask the caller to identify the gender and age of the person that had agonal breathing. The female to male ratio within our dataset was 0.5 and the median age was 62 (IQR: 21). The median duration of a call was 6 minutes 40 seconds (IQR: 2 minutes 47 seconds) (Supplementary Figure \ref{fig:demo}). Each call is rated by the 9-1-1 operator and a quality assurance reviewer with a confidence score indicating the presence of agonal breathing. In order to obtain crisp recordings of agonal breathing, we only train our neural network on audio from calls that are rated with high confidence by both the operator and reviewer. We listened to the remaining 162 calls (19 hours) and manually recorded timestamps where agonal breathing is clearly heard during the call. For every timestamp annotation, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing which translated to 9 minutes 50 seconds of audio.

We train two different models using the same MobileNet architecture and transfer learning technique for the task of a) detecting unwitnessed agonal breathing b) detecting agonal breathing during 9-1-1 calls. The first model is trained with data from Audioset and our second model is trained with non-agonal breathing from our 9-1-1 dataset. We applied k-fold (k=10) cross-validation to the model for detecting unwitnessed agonal breathing and obtained an area under the curve (AUC) of 0.988. We obtain an operating point with an overall sensitivity and specificity of 97.5\% (95\% CI: 94.6 -- 99.1\%) and 95.2\% (95\% CI: 91.6 -- 97.6\%) respectively. We then validate the model for detecting agonal breathing during 9-1-1 calls, and tested it on all 12 hours of non-agonal breathing segments used in 9-1-1 calls that also contained agonal breathing, and which were not used for training and validating the model. Further we only considered pairs of positively marked segments that were sufficiently spaced apart to be indicative of agonal breathing. By applying this heuristic we reduced our false negative rate from 4.5\% to 0.7\%. The sensitivity of this model is 95.3\% (95\% CI: 91.81 -- 97.65\%). Receiver-operating characteristic (ROC) curves were generated to compare the performance of our classifier against each of the eight externally sourced negative classes (Figure \ref{fig:rocs}). 

We benchmark the performance of our model for detecting agonal breathing in several scenarios on an Amazon Echo and an iPhone 5s. In Figure \ref{fig:bm} we show the detection accuracy of our classifier in a domestic setting on a smart speaker and smartphone at different distances of up to 14 feet and when a door separates the speaker and recording device. We test the detection accuracy in the presence of external interfering sounds from our negative dataset played over the air. Finally we show how a smartphone or smartspeaker can use acoustic interference cancellation to reduce the interfering effects of its own audio transmissions (like music) and improve detection accuracy of agonal breathing. 


==> results-2.tex <==

Our dataset consists of recordings of 9-1-1 emergency calls from 2009--2017 provided by Public Health--Seattle \& King County, division of Emergency Medical Services. The dataset includes only calls involving cardiac arrest and specifically those that contained occurrences of agonal breathing. The entire dataset contains 729 calls totaling to 82 hours. The female to male ratio within our dataset was 0.5 and the median age was 62 (IQR: 21). The median duration of a call was 6 minutes 40 seconds (IQR: 2 minutes 47 seconds) (Supplementary Figure \ref{fig:demo}). Each call is rated by the 9-1-1 operator and a quality assurance reviewer with a confidence score indicating the presence of agonal breathing. In order to obtain crisp recordings of agonal breathing, we only train our neural network on audio from calls that are rated with high confidence by both the operator and reviewer. A trained researcher then listened to the remaining 162 calls (19 hours) and manually recorded timestamps where agonal breathing was clearly heard during the call. For every timestamp annotation, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances which translated to 9 minutes 50 seconds of audio.

We trained a convolutional neural network (CNN) to listen to audio signals captured by a smart speaker or smartphone and to output a stream of probabilities that measure the likelihood of agonal breathing in real time. Our system continuously makes predictions on audio segments with a duration of 2.5 seconds which is sufficient for reliably capturing an agonal breath (Figure \ref{fig:sig}A). Each segment is transformed from the time-domain into a spectrogram (Figure \ref{fig:sig}B) which visually represents the power spectral density of the signal, which is the power of each frequency in the audio segment as a function of time. The spectrogram image is then passed into a deep neural network that can distinguish between agonal breathing instances (positive data) and non-agonal instances (negative data). Our classification pipeline of feeding spectrograms into a pretrained convolutional neural network has been shown to be effective for audio classification in prior work\cite{mac2018bat,dennis2011spectrogram,yu2018multi}, in addition to being computationally efficient to train and validate. 
% Recent audio classification systems \cite{oord2016wavenet} use dilated convolutional neural networks 
Our detection algorithm can run in real-time on a smartphone natively and can classify each 2.5 second audio segment within 90 ms. With the smart speaker, the algorithm can run within 145 ms (see materials for how this is estimated).

We train two different models using the MobileNet CNN architecture\cite{mobilenet} that was pre-trained on the ImageNet dataset containing over a 1000 object classes. Using transfer learning\cite{tlearning} we adapt the weights of the CNN to two different tasks. The first task is for the use case of detecting unwitnessed agonal breathing on a smart speaker or a smartphone in a domestic setting. We train a model on negative data from Google's AudioSet\cite{audioset} dataset which contains audio clips from YouTube spanning over 600 audio event classes. We use several non-agonal audio event categories which may be present in a private residence: snoring, ambient noise,  human speech, sounds from a television or radio, cat or dog sounds, fan or air conditioner sounds, coughing and normal breathing. These sounds were selected as we believe they could have a high probability of misclassification. We applied k-fold (k=10) cross-validation to this first model for detecting unwitnessed agonal breathing and obtained an area under the curve (AUC) of 0.995. We obtain an operating point with an overall sensitivity and specificity of 94.1\% (95\% CI: 90.3 -- 96.7\%) and 99.2\% (95\% CI: 98.1 -- 99.7\%) respectively. 

We next generated receiver-operating characteristic (ROC) curves to compare the performance of our classifier against each of the eight externally sourced negative classes (Figure \ref{fig:rocs}). The ROC curve for a given class was generated using k-fold validation. The validation set in each fold was set to contain negative recordings from only a single class to ensure equal class balance between positive and negative recordings. The AUCs for each of the eight negative classes ranged from 0.973 to 0.991.

The second task is for the use case of detecting agonal breathing during a 9-1-1 call. Prior reports have noted that 9-1-1 dispatchers may face challenges identifying agonal breathing during 9-1-1 calls\cite{roppolo2009dispatcher,fukushima2017description}. Our second model is trained with the non-agonal breathing  portions of our dataset of 9-1-1 calls (specific agonal instances are spliced out). We validate the second model for detecting agonal breathing during 9-1-1 calls on 12 hours of non-agonal breathing segments. By relying only on the classifier's probability outputs, we obtain a specificity of 83.4\%. To increase our specificity, we only considered pairs of positively marked segments that were each spaced apart by some time $t$ to be indicative of agonal breathing. We selected $t$ to be within 10 to 20 seconds which is the typical frequency of agonal breathing\cite{roppolo2009dispatcher,lewis2013dispatcher}. This mitigates the effect of spurious false positives. By applying this heuristic we increased our specificity to 99.8\%. The sensitivity of our classifier without this heuristic is 93\% (95\% CI: 89.73 -- 96.40\%). We note that the sensitivity obtained by applying this heuristic would not accurately reflect our detection rate in a practical deployment on a smart speaker system. This is due to the nature of our dataset, wherein agonal breathing is predominantly heard for a short period of time when the operator instructs the witness to hold the phone close to the victim. Additionally some of our calls only contain a single obvious agonal breath, and this heuristic would not detect them. In our proposed use case a static smart speaker or smartphone would pick up on the entire duration of agonal breathing which has been estimated to last for approximately 4 minutes \cite{roppolo2009dispatcher} in the early phase of cardiac arrest.

%Another important concern is the issue of potential false positives, given that a true positive classification should lead to activation of the emergency response system. Put differently, having a low false positive rate would be critical to manage appropriately public resources and avoid unnecessary deployment of EMS. To further explore how to mitigate false-positives, we ran our model trained on Google's AudioSet on 20 hours of audio of ambient sound from a single person in a private residence.\cite{sitting}. By relying on the classifier's probabilities alone, we obtain a false positive rate of 0.0034\% (1 false positive across the entire stream). We then ran the model on 20 continuous hours of Google's AudioSet snoring sounds. Using the classifier's probabilities alone we obtain a false positive rate of 3.97\%. To reduce false positives, we implement a heuristic that classifies segments as agonal if the frequency is consistent with agonal breathing patterns observed in a prior report (i.e., within a range of 3 to 6 times a minutes\cite{roppolo2009dispatcher}). Tracking the pattern of positive audio segments for up to 20 seconds reduces the false positive rate to 0.34\% and waiting for up to 60 seconds reduces the false positive rate to 0\%. Additional agonal instances could help improve the specificity further, which would be required for a real-world implementation. A real-world implementation would also require a user-interface that has a confirmatory/cancellation opportunity before the emergency medical response system was activated.

We next visually investigate the features learned by our neural network. First, we used LIME\cite{lime} to highlight the regions of a spectrogram that contribute most to the neural network's predictions. Figure \ref{fig:sig}C shows a masked spectrogram of agonal breathing. There is a correlation between the regions where agonal breathing occurs and the pixels that the classifier deems most important. Second, we applied t-SNE\cite{tsne} to visualize the high-dimensional outputs of the CNN's final hidden layer by projecting the features into the 2-D space (Figure \ref{fig:sig}D). The two clusters represent the abstract features of the agonal breathing and non-agonal breathing spectrograms for a subset of the non-agonal breathing sounds.

We next benchmark the performance of our model for detecting agonal breathing in several scenarios on an Amazon Echo and an Apple iPhone 5s. For these experiments we played the 236 audio clips of agonal breathing from an external speaker and captured the audio on the Echo and smartphone. In Figure \ref{fig:bm} we show the detection accuracy of our classifier in a domestic setting on a smart speaker and smartphone. Figure \ref{fig:bm}A shows the detection accuracy of our classifier at distances of 1, 3, 6, 9, 12 and 14 meters on the Echo and iPhone 5s. Both devices achieve close to ideal detection across distances of 1 to 6 meters. At a distance of 14 meters, the Echo and smartphone have a detection accuracy of 78.4\% $\pm$ 5.8\% and 91.6\% $\pm$ 6.72\% respectively. Figure \ref{fig:bm}B shows detection accuracies when a door separates the speaker and recording device. The detection accuracy is $>$ 95\% for both devices at distances of 1 to 3 meters. Detection accuracies drop off quickly and the audio clips are close to undetectable at 14 meters. The range of 1 -- 3 meters may be sufficient in situations where the agonal breathing event and recording device are in adjacent rooms such as a bedroom and ensuite bathroom. We also evaluated the effect of placing the smartphone in a pocket, with the subject supine on the ground and the speaker next to the head, and obtain a detection accuracy of 97.4\% $\pm$ 3.5\%. Figure \ref{fig:bm}C shows our system performance, using the same experimental setup, but in the presence of 5 classes of interfering sounds, namely fan and air conditioner sounds, human speech, cat and dog sounds, music and shower sounds. The interfering sounds and the agonal breathing sounds are played from separate speakers that are placed 3 meters away from the recording devices and perpendicular to each other. The interfering noise is played at a similar volume to the agonal breathing recordings. Across all interfering sound classes the smart speaker and smartphone both achieve a detection accuracy of at least 91\%. Finally we evaluate how a smartphone or smartspeaker can use acoustic interference cancellation to reduce the interfering effects of its own audio transmissions (like music) and improve detection accuracy of agonal breathing (Figure \ref{fig:bm}D). We set the smartphone to play music at a louder volume than the agonal breathing audio clips, while simultaneously recording audio of the agonal breathing. Without any audio cancellation, the detection accuracy is consistently poor, with an average accuracy of 9.5\% across distances. When the audio cancellation algorithm is applied, our detection accuracy improves to 97.0\% $\pm$ 3.4\% at a distance of 1 meter, and gradually decreases to an accuracy of 74.9\% $\pm$ 15.4\% at 14 meters.


==> results-3.tex <==

Our dataset consists of recordings of 9-1-1 emergency calls from 2009--2017 provided by Public Health--Seattle \& King County, division of Emergency Medical Services. The dataset includes only calls involving cardiac arrest and specifically those that contained occurrences of agonal breathing. The entire dataset contains 729 calls totaling to 82 hours. The female to male ratio within our dataset was 0.5 and the median age was 62 (interquartile range (IQR): 21). The median duration of a call was 6 minutes 40 seconds (IQR: 2 minutes 47 seconds) (Supplementary Figure \ref{fig:demo}). Each call is rated by the 9-1-1 operator and a quality assurance reviewer with a confidence score indicating the presence of agonal breathing. In order to obtain crisp recordings of agonal breathing, we only train our neural network on audio from calls that are rated with high confidence by both the operator and reviewer. A trained researcher then listened to the remaining 162 calls (19 hours) and manually recorded timestamps where agonal breathing was clearly heard during the call. For every timestamp annotation, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances which translated to 9 minutes 50 seconds of audio.

We trained a convolutional neural network (CNN) to listen to audio signals captured by a smart speaker or smartphone and to output a stream of probabilities that measure the likelihood of agonal breathing in real-time. Our system continuously makes predictions on audio segments with a duration of 2.5 seconds which is sufficient for reliably capturing an agonal breath (Figure \ref{fig:sig}A). Each segment is transformed from the time-domain into a spectrogram (Figure \ref{fig:sig}B) which visually represents the power spectral density of the signal, which is the power of each frequency in the audio segment as a function of time. The spectrogram image is then passed into a deep neural network that can distinguish between agonal breathing instances (positive data) and non-agonal instances (negative data). Our classification pipeline of feeding spectrograms into a pretrained convolutional neural network has been shown to be effective for audio classification in prior work\cite{mac2018bat,dennis2011spectrogram,yu2018multi}, in addition to being computationally efficient to train and validate. 
% Recent audio classification systems \cite{oord2016wavenet} use dilated convolutional neural networks 
Our detection algorithm can run in real-time on a smartphone natively and can classify each 2.5 second audio segment within 90 ms. With the smart speaker, the algorithm can run within 145 ms (see materials for how this is estimated).

We train two different models using the MobileNet CNN architecture\cite{mobilenet} that was pre-trained on the ImageNet dataset containing over a 1000 object classes. Using transfer learning\cite{tlearning} we adapt the weights of the CNN to two different tasks. The first task is for the use case of detecting unwitnessed agonal breathing on a smart speaker or a smartphone in a domestic setting. We train a model on negative data from Google's AudioSet\cite{audioset} dataset which contains audio clips spanning over 600 audio event classes. We use several non-agonal audio event categories which may be present in a private residence: snoring, ambient noise,  human speech, sounds from a television or radio, cat or dog sounds, fan or air conditioner sounds, coughing and normal breathing. These sounds were selected as we believe they could have a high probability of misclassification. We applied k-fold (k=10) cross-validation to this first model for detecting unwitnessed agonal breathing and obtained an area under the curve (AUC) of 0.995. We obtain an operating point with an overall sensitivity and specificity of 94.1\% (95\% CI: 90.3 -- 96.7\%) and 99.2\% (95\% CI: 98.1 -- 99.7\%) respectively. 

We next generated receiver-operating characteristic (ROC) curves to compare the performance of our classifier against each of the eight externally sourced negative classes (Figure \ref{fig:rocs}). The ROC curve for a given class was generated using k-fold validation. The validation set in each fold was set to contain negative recordings from only a single class to ensure equal class balance between positive and negative recordings. The AUCs for each of the eight negative classes ranged from 0.991 to 0.999.

The second task is for the use case of detecting agonal breathing during a 9-1-1 call. Prior reports have noted that 9-1-1 dispatchers may face challenges identifying agonal breathing during 9-1-1 calls, leading to delays in CPR\cite{roppolo2009dispatcher,fukushima2017description,blomberg2018}. We validate our model using 10 hours of non-agonal breathing segments from the 9-1-1 cardiac arrest calls. By relying only on the classifier's probability outputs, we obtain a specificity of 99.7\%. To increase our specificity, we only considered pairs of positively marked segments that were each spaced apart by some time $t$ to be indicative of agonal breathing. We selected $t$ to be within 10 to 20 seconds which is the typical frequency of agonal breathing\cite{roppolo2009dispatcher,lewis2013dispatcher}. This mitigates the effect of spurious false positives. By applying this heuristic we increased our specificity to 99.99\%. We note that the sensitivity obtained by applying this heuristic would not accurately reflect our detection rate in a practical deployment on a smart speaker system. This is due to the nature of our dataset, wherein agonal breathing is predominantly heard for a short period of time when the operator instructs the witness to hold the phone close to the victim. Additionally some of our calls only contain a single obvious agonal breath, and this heuristic would not detect them. In our proposed use case a static smart speaker or smartphone would pick up on the entire duration of agonal breathing which has been estimated to last for approximately 4 minutes \cite{roppolo2009dispatcher} in the early phase of cardiac arrest.

% Another important concern is the issue of potential false positives, given that a true positive classification should lead to activation of the emergency response system. Put differently, having a low false positive rate would be critical to manage appropriately public resources and avoid unnecessary deployment of EMS. To further explore how to mitigate false-positives, we ran our model trained on Google's AudioSet on 20 hours of audio of ambient sound from a single person in a private residence.\cite{sitting}. By relying on the classifier's probabilities alone, we obtain a false positive rate of 0.0034\% (1 false positive across the entire stream). We then ran the model on 20 continuous hours of Google's AudioSet snoring sounds. Using the classifier's probabilities alone we obtain a false positive rate of 3.97\%. To reduce false positives, we implement a heuristic that classifies segments as agonal if the frequency is consistent with agonal breathing patterns observed in a prior report (i.e., within a range of 3 to 6 times a minutes\cite{roppolo2009dispatcher}). Tracking the pattern of positive audio segments for up to 20 seconds reduces the false positive rate to 0.34\% and waiting for up to 60 seconds reduces the false positive rate to 0\%. Additional agonal instances could help improve the specificity further, which would be required for a real-world implementation. A real-world implementation would also require a user-interface that has a confirmatory/cancellation opportunity before the emergency medical response system was activated.

We next visually investigate the features learned by our neural network. First, we used LIME\cite{lime} to highlight the regions of a spectrogram that contribute most to the neural network's predictions. Figure \ref{fig:sig}C shows a masked spectrogram of agonal breathing. There is a correlation between the regions where agonal breathing occurs and the pixels that the classifier deems most important. Second, we applied t-SNE\cite{tsne} to visualize the high-dimensional outputs of the CNN's final hidden layer by projecting the features into the 2-D space (Figure \ref{fig:sig}D). The two clusters represent the abstract features of the agonal breathing and non-agonal breathing spectrograms for a subset of the non-agonal breathing sounds.

We next benchmark the performance of our model for detecting agonal breathing in several scenarios on an Amazon Echo and an Apple iPhone 5s. For these experiments we played the 236 audio clips of agonal breathing from an external speaker and captured the audio on the Echo and smartphone. In Figure \ref{fig:bm} we show the detection accuracy of our classifier in a domestic setting on a smart speaker and smartphone. Figure \ref{fig:bm}A shows the detection accuracy of our classifier at distances of 1, 3, 6, 9, 12 and 14 meters on the Echo and iPhone 5s. Both devices achieve close to ideal detection across distances of 1 to 6 meters. At a distance of 14 meters, the Echo and smartphone have a detection accuracy of 78.4\% $\pm$ 5.8\% and 91.6\% $\pm$ 6.72\% respectively. Figure \ref{fig:bm}B shows detection accuracies when a door separates the speaker and recording device. The detection accuracy is $>$ 95\% for both devices at distances of 1 to 3 meters. Detection accuracies drop off quickly and the audio clips are close to undetectable at 14 meters. The range of 1 -- 3 meters may be sufficient in situations where the agonal breathing event and recording device are in adjacent rooms such as a bedroom and ensuite bathroom. We also evaluated the effect of placing the smartphone in a pocket, with the subject supine on the ground and the speaker next to the head, and obtain a detection accuracy of 97.4\% $\pm$ 3.5\%. Figure \ref{fig:bm}C shows our system performance, using the same experimental setup, but in the presence of 5 classes of interfering sounds, namely fan and air conditioner sounds, human speech, cat and dog sounds, music and shower sounds. The interfering sounds and the agonal breathing sounds are played from separate speakers that are placed 3 meters away from the recording devices and perpendicular to each other. The interfering noise is played at a similar volume to the agonal breathing recordings. Across all interfering sound classes the smart speaker and smartphone both achieve a detection accuracy of at least 91\%. Finally we evaluate how a smartphone or smartspeaker can use acoustic interference cancellation to reduce the interfering effects of its own audio transmissions (like music) and improve detection accuracy of agonal breathing (Figure \ref{fig:bm}D). We set the smartphone to play music at a louder volume than the agonal breathing audio clips, while simultaneously recording audio of the agonal breathing. Without any audio cancellation, the detection accuracy is consistently poor, with an average accuracy of 9.5\% across distances. When the audio cancellation algorithm is applied, our detection accuracy improves to 97.0\% $\pm$ 3.4\% at a distance of 1 meter, and gradually decreases to an accuracy of 74.9\% $\pm$ 15.4\% at 14 meters.


==> results-4.tex <==

Our agonal breathing recordings are sourced from 9-1-1 emergency calls from 2009--2017, provided by Public Health--Seattle \& King County, Division of Emergency Medical Services. The dataset included 162 calls (19 hours) that had clear recordings of agonal breathing. These instances predominantly occur when the 9-1-1 operator asked the caller to place the phone next to the victim's mouth for the purposes of breathing identification. For each occurrence, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances. Our negative dataset consists of 83 hours of audio data captured during polysomnographic sleep studies, across 12 different patients and includes instances of hypopnea, central apnea, obstructive apnea, snoring and breathing. The negative dataset also includes interfering sounds that might be played in a bedroom while a person is asleep, specifically a podcast, sleep soundscape and white noise.

% We trained a SVM for the use case of detecting unwitnessed agonal breathing on a smart speaker or a smartphone in a domestic setting when the victim is in a bedroom and sleeping. 
Our model includes audio signals captured by a smart speaker or smartphone and outputs the probability of agonal breathing in real-time on each 2.5s audio segment. We use Google's VGGish model\cite{vggish} as a feature extractor to transform the raw audio waveforms into embeddings which are passed into the SVM. Each segment is transformed from the time-domain into a log-mel spectrogram\cite{muda2010voice}, and is further compressed into a feature embedding using principal component analysis. These embeddings are then passed into an SVM with a radial basis function kernel that can distinguish between agonal breathing instances (positive data) and non-agonal instances (negative data) (Figure \ref{fig:pipeline}A).
Given the relatively small size of our agonal breathing dataset, we augmented the number of agonal breathing instances with label preserving transformations, a common technique applied to sparse datasets\cite{cui2015data,wong2016understanding} (see methods and material). Figures \ref{fig:pipeline}B,C show example audio waveforms and spectrograms for agonal breathing, snoring and apnea events.

% \textcolor{red}{Finally, the classifier's predictions are passed into a timing detector that checks if the rate of positive predictions is within the typical frequency in which agonal breathing occurs .}
% {SHYAM: IS this last line done for the specificity and sensitivity cross-validation?}
% Justin: No, that is only for the FPR analysis, we don't have a stream to apply this to to get sensitivity numbers, only specificity numbers


We applied k-fold (k=10) cross-validation and obtained an area under the curve (AUC) of 0.998 $\pm$ 0.003 (Figure \ref{fig:result}A). We obtain an operating point with an overall sensitivity and specificity of 98.51\% (95\% CI: 98.21 -- 98.78\%) and 98.05\% (95\% CI: 97.71 -- 98.35\%) respectively (Figure \ref{fig:result}B). Our detection algorithm can run in real-time on a smartphone natively and can classify each 2.5 second audio segment within 106 ms. With the smart speaker, the algorithm can run within 660 ms. We visualized the audio embeddings of our dataset by using t-SNE\cite{tsne} to project the features into the 2-D space (Figure \ref{fig:result}C). The two clusters represent the abstract features of agonal breathing instances and audio from the polysomnographic studies.

 To evaluate false positive rate, we run our classifier over the full 83 hour audio stream collected in the sleep lab. By relying only on the classifier's probability outputs, we obtain a false positive rate of 0.121\%, this corresponds to 145 of 119,425 audio segments. To reduce false positives, the classifier's predictions are passed through a frequency filter that checks if the rate of positive predictions is within the typical frequency at which agonal breathing occurs (i.e., within a range of 3 to 6 agonal breaths per minute\cite{roppolo2009dispatcher,lewis2013dispatcher}). This reduced the false positive rate to 0\%, when considering agonal breathing within a duration of 10-20s. In our proposed use case a static smart speaker or smartphone would be able to operate on the entire duration of agonal breathing which has been estimated to last for approximately 4 minutes, \cite{roppolo2009dispatcher} in the early phase of cardiac arrest.

We next benchmark the performance of our model.  For these experiments we played the audio clips of agonal breathing over air from an external speaker and captured the audio on an Amazon Echo and Apple iPhone 5s. In Figure \ref{fig:bm} we show the detection accuracy of our classifier in a domestic setting on a smart speaker and smartphone. We evaluate detection accuracy using the k=10 validation folds in our dataset such that no audio file in the validation set appears in any of the different recording conditions in the training set. Figure \ref{fig:bm}A shows the detection accuracy of our classifier in ambient conditions at distances of 1, 3, and 6 meters on the Echo and iPhone 5s. Both devices achieve greater than 99\% mean accuracy at distances up to 3 meters. We also evaluated the effect of placing the smartphone in a pocket, with the subject supine on the ground and the speaker next to the head, and obtain a mean detection accuracy of 97.00\% $\pm$ 3.32\%. Figure \ref{fig:bm}B shows our system performance, using the same experimental setup, but in the presence of indoor interfering sounds (cat, dog, air conditioner) and outdoor interfering sounds (traffic, construction and human speech). Across all interfering sound classes the smart speaker and smartphone achieve a mean detection accuracy of 98.5\%. Finally we evaluate how a smartphone or smartspeaker can use acoustic interference cancellation to reduce the interfering effects of its own audio transmissions and improve detection accuracy of agonal breathing (Figure \ref{fig:bm}C,D). We set the smartphone to play sounds one might play to fall asleep including a podcast, sleep soundscape (i.e., river current) and white noise. We play them at a soft (45 dBA) and loud (67 dBA) volume. Simultaneously we play the agonal breathing audio clips. Without any audio cancellation, the detection accuracy is consistently poor, with an average accuracy of 12.16\% and 1.92\% across distances and sounds for soft and loud interfering volumes. When the audio cancellation algorithm is applied, our detection accuracy achieves an average accuracy of 98.91\% and 98.51\% across distances and sounds for soft and loud interfering volumes respectively.


==> results-5.tex <==

Our agonal breathing recordings are sourced from 9-1-1 emergency calls from 2009--2017, provided by Public Health--Seattle \& King County, Division of Emergency Medical Services. The dataset included 162 calls (19 hours) that had clear recordings of agonal breathing. These instances predominantly occur when the 9-1-1 operator asked the caller to place the phone next to the victim's mouth for the purposes of breathing identification. For each occurrence, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances. \red{These clips are played over the air at different distances, in the presence of interfering sounds, in a pocket and at different volumes and recorded on different devices to get 7316 samples.} Our negative dataset consists of 83 hours of audio data captured during polysomnographic sleep studies, across 12 different patients and includes instances of hypopnea, central apnea, obstructive apnea, snoring and breathing. The negative dataset also includes interfering sounds that might be played in a bedroom while a person is asleep, specifically a podcast, sleep soundscape and white noise. \red{One hour of snoring and the interfering sounds are played over the air at different distances and recorded on different devices to get 7339 samples.} 

% We trained a SVM for the use case of detecting unwitnessed agonal breathing on a smart speaker or a smartphone in a domestic setting when the victim is in a bedroom and sleeping. 
Our model includes audio signals captured by a smart speaker or smartphone and outputs the probability of agonal breathing in real-time on each 2.5s audio segment. We use Google's VGGish model\cite{vggish} as a feature extractor to transform the raw audio waveforms into embeddings which are passed into the SVM. Each segment is transformed from the time-domain into a log-mel spectrogram\cite{muda2010voice}, and is further compressed into a feature embedding using principal component analysis. These embeddings are then passed into an SVM with a radial basis function kernel that can distinguish between agonal breathing instances (positive data) and non-agonal instances (negative data) (Figure \ref{fig:pipeline}A).
Given the relatively small size of our agonal breathing dataset, we augmented the number of agonal breathing instances with label preserving transformations, a common technique applied to sparse datasets\cite{cui2015data,wong2016understanding} (see methods and material). Figures \ref{fig:pipeline}B,C show example audio waveforms and spectrograms for agonal breathing, snoring and apnea events.

% \textcolor{red}{Finally, the classifier's predictions are passed into a timing detector that checks if the rate of positive predictions is within the typical frequency in which agonal breathing occurs .}
% {SHYAM: IS this last line done for the specificity and sensitivity cross-validation?}
% Justin: No, that is only for the FPR analysis, we don't have a stream to apply this to to get sensitivity numbers, only specificity numbers

We applied k-fold (k=10) cross-validation and obtained an area under the curve (AUC) of 0.998 $\pm$ 0.004 (Figure \ref{fig:result}A). We obtain an operating point with an overall sensitivity and specificity of 97.03\% (95\% CI: 96.62 -- 97.41\%) and 98.20\% (95\% CI: 97.87 -- 98.49\%) respectively (Figure \ref{fig:result}B). Our detection algorithm can run in real-time on a smartphone natively and can classify each 2.5 second audio segment within 21 ms. With the smart speaker, the algorithm can run within 58 ms. We visualized the audio embeddings of our dataset by using t-SNE\cite{tsne} to project the features into the 2-D space (Figure \ref{fig:result}C). The two clusters represent the abstract features of agonal breathing instances and audio from the polysomnographic studies.

To evaluate false positive rate, we run our classifier over the full audio stream collected in the sleep lab. The sleep audio used to train the model was excluded from evaluation. By relying only on the classifier's probability outputs, we obtain a false positive rate of 0.1009\%, this corresponds to 119 of 117,985 audio segments. To reduce false positives, the classifier's predictions are passed through a frequency filter that checks if the rate of positive predictions is within the typical frequency at which agonal breathing occurs (i.e., within a range of 3 to 6 agonal breaths per minute\cite{roppolo2009dispatcher,lewis2013dispatcher}). This reduced the false positive rate to 0.0025\%, when considering agonal breathing within a duration of 10-20s. The filter can be applied again to reduce the false positive rate to 0\%. In our proposed use case a static smart speaker or smartphone would be able to operate on the entire duration of agonal breathing which has been estimated to last for approximately 4 minutes, \cite{roppolo2009dispatcher} in the early phase of cardiac arrest.

We next benchmark the performance of our model.  For these experiments we played the audio clips of agonal breathing over air from an external speaker and captured the audio on an Amazon Echo and Apple iPhone 5s. In Figure \ref{fig:bm} we show the detection accuracy of our classifier in a domestic setting on a smart speaker and smartphone. We evaluate detection accuracy using the k=10 validation folds in our dataset such that no audio file in the validation set appears in any of the different recording conditions in the training set. Figure \ref{fig:bm}A shows the detection accuracy of our classifier in ambient conditions at distances of 1, 3, and 6 meters on the Echo and iPhone 5s. Both devices achieve greater than 98.7\% mean accuracy at distances up to 3 meters. We also evaluated the effect of placing the smartphone in a pocket, with the subject supine on the ground and the speaker next to the head, and obtain a mean detection accuracy of 92.31\% $\pm$ 6.11\%. Figure \ref{fig:bm}B shows our system performance, using the same experimental setup, but in the presence of indoor interfering sounds (cat, dog, air conditioner) and outdoor interfering sounds (traffic, construction and human speech). Across all interfering sound classes the smart speaker and smartphone achieve a mean detection accuracy of 96.95\%. Finally we evaluate how a smartphone or smartspeaker can use acoustic interference cancellation to reduce the interfering effects of its own audio transmissions and improve detection accuracy of agonal breathing (Figure \ref{fig:bm}C,D). We set the smartphone to play sounds one might play to fall asleep including a podcast, sleep soundscape (i.e., river current) and white noise. We play them at a soft (45 dBA) and loud (67 dBA) volume. Simultaneously we play the agonal breathing audio clips. Without any audio cancellation, the detection accuracy is consistently poor, with an average accuracy of 11.84\% and 3.82\% across distances and sounds for soft and loud interfering volumes. When the audio cancellation algorithm is applied, our detection accuracy achieves an average accuracy of 97.60\% and 95.41\% across distances and sounds for soft and loud interfering volumes respectively.


==> results-npj.tex <==

Our agonal breathing recordings are sourced from 9-1-1 emergency calls from 2009--2017, provided by Public Health--Seattle \& King County, Division of Emergency Medical Services. The dataset included 162 calls (19 hours) that had clear recordings of agonal breathing. For each occurrence, we extract 2.5 seconds worth of audio from the start of each agonal breath. We extracted a total of 236 clips of agonal breathing instances. {We augment the number of agonal breathing instances with label preserving transformations, a common technique applied to sparse datasets\cite{cui2015data,wong2016understanding}. We augment the data by playing the recordings over the air over distances of 1, 3 and 6 meters, in the presence of interference from indoor and outdoor sounds with different volumes and when a noise cancellation filter is applied. The recordings were captured on different devices, namely an Amazon Alexa, an iPhone 5s and a Samsung Galaxy S4 to get 7316 positive samples.} Our negative dataset consists of 83 hours of audio data captured during polysomnographic sleep studies, across 12 different patients and includes instances of hypopnea, central apnea, obstructive apnea, snoring and breathing. The negative dataset also includes interfering sounds that might be played in a bedroom while a person is asleep, specifically a podcast, sleep soundscape and white noise. {To train our model, we use one hour of audio data from the  sleep study as well as the other interfering sounds. These audio signals were played over the air at different distances and recorded on different devices to get 7339 samples. The remaining 82 hours of sleep data (117,895 audio segments) is then used for validating the performance of our model.} 

% We trained a SVM for the use case of detecting unwitnessed agonal breathing on a smart speaker or a smartphone in a domestic setting when the victim is in a bedroom and sleeping. 
Our model includes audio signals captured by a smart speaker or smartphone and outputs the probability of agonal breathing in real-time on each 2.5s audio segment. We use Google's VGGish model\cite{vggish} as a feature extractor to transform the raw audio waveforms into embeddings which are passed into the SVM. Each segment is transformed from the time-domain into a log-mel spectrogram\cite{muda2010voice}, and is further compressed into a feature embedding using principal component analysis. These embeddings are then passed into an SVM with a radial basis function kernel that can distinguish between agonal breathing instances (positive data) and non-agonal instances (negative data) (Figure \ref{fig:result}A).
Given the relatively small size of our agonal breathing dataset, we augmented the number of agonal breathing instances with label preserving transformations, a common technique applied to sparse datasets\cite{cui2015data,wong2016understanding} (see methods and material). Supplementary Figure \ref{fig:sig}A,B show example audio waveforms and spectrograms for agonal breathing, snoring and apnea events.

% \textcolor{red}{Finally, the classifier's predictions are passed into a timing detector that checks if the rate of positive predictions is within the typical frequency in which agonal breathing occurs .}
% {SHYAM: IS this last line done for the specificity and sensitivity cross-validation?}
% Justin: No, that is only for the FPR analysis, we don't have a stream to apply this to to get sensitivity numbers, only specificity numbers

\subsection*{Classifier Performance}
We applied k-fold (k=10) cross-validation and obtained an area under the curve (AUC) of 0.998 $\pm$ 0.004 (Figure \ref{fig:result}B). We obtain an operating point with an overall sensitivity and specificity of 97.03\% (95\% CI: 96.62 -- 97.41\%) and 98.20\% (95\% CI: 97.87 -- 98.49\%) respectively (Figure \ref{fig:result}C). Our detection algorithm can run in real-time on a smartphone natively and can classify each 2.5 second audio segment within 21 ms. With the smart speaker, the algorithm can run within 58 ms. We visualized the audio embeddings of our dataset by using t-SNE\cite{tsne} to project the features into the 2-D space (Figure \ref{fig:result}D). The two clusters represent the abstract features of agonal breathing instances and audio from the polysomnographic studies.

To evaluate false positive rate, we run our classifier over the full audio stream collected in the sleep lab. The sleep audio used to train the model was excluded from evaluation. By relying only on the classifier's probability outputs, we obtain a false positive rate of 0.1009\%, this corresponds to 119 of 117,985 audio segments. To reduce false positives, the classifier's predictions are passed through a frequency filter that checks if the rate of positive predictions is within the typical frequency at which agonal breathing occurs (i.e., within a range of 3 to 6 agonal breaths per minute\cite{roppolo2009dispatcher,lewis2013dispatcher}). This reduced the false positive rate to 0.0025\%, when considering two agonal breaths within a duration of 10-20s. When considering three agonal breaths within the same duration, the false positive rate reduces to 0\% (Figure \ref{fig:result}E). In our proposed use case a static smart speaker or smartphone would be able to operate on the entire duration of agonal breathing which has been estimated to last for approximately 4 minutes, \cite{roppolo2009dispatcher} in the early phase of cardiac arrest.

\subsection*{Benchmark Performance}
We next benchmark the performance of our model.  For these experiments we played the audio clips of agonal breathing over air from an external speaker and captured the audio on an Amazon Echo and Apple iPhone 5s. In Figure \ref{fig:bm} we show the detection accuracy of our classifier in a domestic setting on a smart speaker and smartphone. We evaluate detection accuracy using the k=10 validation folds in our dataset such that no audio file in the validation set appears in any of the different recording conditions in the training set. Figure \ref{fig:bm}A shows the detection accuracy of our classifier in ambient conditions at distances of 1, 3, and 6 meters on the Echo and iPhone 5s. Both devices achieve greater than 98.7\% mean accuracy at distances up to 3 meters. We also evaluated the effect of placing the smartphone in a pocket, with the subject supine on the ground and the speaker next to the head, and obtain a mean detection accuracy of 92.31\% $\pm$ 6.11\%. Figure \ref{fig:bm}B shows our system performance, using the same experimental setup, but in the presence of indoor interfering sounds (cat, dog, air conditioner) and outdoor interfering sounds (traffic, construction and human speech). Across all interfering sound classes the smart speaker and smartphone achieve a mean detection accuracy of 96.95\%. Finally we evaluate how a smartphone or smartspeaker can use acoustic interference cancellation to reduce the interfering effects of its own audio transmissions and improve detection accuracy of agonal breathing (Figure \ref{fig:bm}C,D). We set the smartphone to play sounds one might play to fall asleep including a podcast, sleep soundscape (i.e., river current) and white noise. We play them at a soft (45 dBA) and loud (67 dBA) volume. Simultaneously we play the agonal breathing audio clips. Without any audio cancellation, the detection accuracy is consistently poor, with an average accuracy of 11.84\% and 3.82\% across distances and sounds for soft and loud interfering volumes. When the audio cancellation algorithm is applied, our detection accuracy achieves an average accuracy of 97.60\% and 95.41\% across distances and sounds for soft and loud interfering volumes respectively.


